Convex Computation of the Reachable Set for Hybrid Systems with Parametric Uncertainty

To verify the correct operation of systems, engineers need to determine the set of configurations of a dynamical model that are able to safely reach a specified configuration under a control law. Unfortunately, constructing models for systems interacting in highly dynamic environments is difficult. This paper addresses this challenge by presenting a convex optimization method to efficiently compute the set of configurations of a polynomial hybrid dynamical system that are able to safely reach a user defined target set despite parametric uncertainty in the model. This class of models describes, for example, legged robots moving over uncertain terrains. The presented approach utilizes the notion of occupation measures to describe the evolution of trajectories of a nonlinear hybrid dynamical system with parametric uncertainty as a linear equation over measures whose supports coincide with the trajectories under investigation. This linear equation with user defined support constraints is approximated with vanishing conservatism using a hierarchy of semidefinite programs that are each proven to compute an inner/outer approximation to the set of initial conditions that can reach the user defined target set safely in spite of uncertainty. The efficacy of this method is illustrated on a collection of six representative examples.

==> sections/sec_app_dual.tex <==
\section{Calculations for the dual}
\label{app:dual_exp}
For simplicity, we only consider one mode system with one guard that resets back into the same mode. A more general version follows as a direct extension.\par
The Liouville eqn. of interest for any test function $v\in C(\mathcal T\times D\times \Theta)$ is the following
\begin{flalign}
\begin{split}
\ip{\mu_0,\ip{v(0,\cdot,\cdot),\mu_\theta}} +\ip{\sigma,\ip{v,\mu_\theta}} +\ip{\mathcal L_f'\mu,v}\\
=\ip{\delta_T\times \mu_T,v}+\ip{\mu_{G_{(1,1)}},v}
\end{split}
\label{eq:1}
\end{flalign}
Let $r(t,x):=\ip{\mu_\theta,v}$ and recall that $\sigma := R_{(1,1)}^*\pi_{(t,x_1)}^*\mu_G$, where $\pi_{(t,x)}^*\mu_G$ is the $(t,x)$ marginal of $\mu_G$.
Thus,
\begin{align}
\ip{\sigma,r}=\ip{\pi_{(t,x)}^*\mu_{G_{(1,1)}},r(t,R_{(1,1)}(x))}
\end{align}
By definition of the marginal
\begin{flalign}
&&\ip{\mu_{G_{(1,1)}},s}=&\,\ip{\pi_{(t,x_1)}^*\mu_{G_{(1,1)}},s}&\forall s\in C(\mathcal T\times D)
\end{flalign}
and the fact that $R^{-1}_{(1,1)}(\Sigma)=spt(\pi_{(t,x)}^*\mu_G)$, it follows that
\begin{align}
\ip{\sigma,r}=\ip{\mu_{G_{(1,1)}},r(t,R_{(1,1)}(x))}
\label{eq:2}
\end{align}
From Eqn.~(\ref{eq:2}), Eqn.~(\ref{eq:1}) simplifies to
\begin{align}
\begin{split}
\ip{\mu_0,\ip{v(0,\cdot,\cdot),\mu_\theta}}+\ip{\mathcal L_f'\mu,v}\\
=\ip{\mu_T,v(T,\cdot,\cdot)}+\ip{\mu_{G_{(1,1)}},v-\ip{v,\mu_\theta}}
\end{split}
\end{align}


==> sections/sec_app_overlap.tex <==
\section{Commentary on Assumption~\ref{assum:overlap}}
\label{sec:overlap}
\begin{prop}
  blah
\end{prop} 

==> sections/sec_confidence.tex <==
\section{Estimates of BRS with $\alpha$-confidence} 
The last section addressed the case wherein the goal was to estimate the set of initial conditions (state) were independent of parameters (read uncertainties drawn from a distribution $\mu_{\theta_j}$) that reaches a certain terminal set $X_T$ . Clearly, for one initial condition and a given $\mu_{\theta_j}$, the distribution of terminal states is related to the advection of $\mu_{\theta_j}$ along the ow of the state trajectories. By extension, given a set of initial conditions, the set of terminal states is going to be distributed over a set, not necessarily uniformly.
In this section, we attempt to identify the set of initial conditions that can guarantee that the terminal state lies in $\mathcal X_T$ with some $\alpha $ confidence.
\par
To that end, we redefine one of the measures of interest -- the terminal measure:
\begin{align}
\mu_T(A\times B)=\int_{\mathcal X\times \Theta} I_{A\times B}(x(T\mid x_0,\theta_0),\theta(T\mid \theta_0))\,d\,\mu_0\times \mu_\theta	
\end{align}
only this time, $\mu_T\in \mathcal M(\mathcal X\times \Theta)$ as opposed to the last section wherein $\mu_T\in \mathcal M(\mathcal X_T\times \Theta)$. With this redefinition, the primal problem is as stated in the following.
\begin{flalign}
	\sup \ip{\mu_0,1}\\
	&&\delta_T\otimes(\mu_{T_1}+\mu_{T_2})=&\,\delta_0\otimes\mu_0\otimes \mu_\theta+\mathcal L_{\tilde f}'\mu&\\
	&& \mu_0+\hat\mu_0=&\,\lambda\\
	&& \alpha\ip{\mu_{T_1}+\mu_{T_2},1}+r=&\,\ip{\mu_{T_1},1}
\end{flalign}
where $\mu_{T_1}\in \mathcal M(\mathcal X_T\times \Theta), \mu_{T_2}\in \mathcal M(\mathcal X\backslash \mathcal X_T\times \Theta),\mu_0,\hat \mu_0\in \mathcal M(\mathcal X)$ and $r\in \R_{\ge 0}$.\\
The dual to the above reads as follows
\begin{flalign}
\inf \ip{\lambda,w}\\
&& w\ge &\,0&\\
&& v(T,\cdot,\cdot)+q(\alpha-1)\ge&\, 0 & \forall (x,\theta)\in \mathcal X_T\times \Theta\\
&& v(T,\cdot,\cdot)+q\alpha\ge&\, 0 & \forall (x,\theta)\in \mathcal X\times \Theta\backslash\mathcal X_T\times \Theta\\
&& - \mathcal L_{\tilde f}v\ge&\,0 & \forall (x,\theta)\in \mathcal X\times \Theta\\
&& w-1-\int_\Theta v(0,\cdot,\theta)\,d\mu_\theta(\theta)\ge &\,0 & \forall x\in \mathcal X
\end{flalign}
where $v\in C^1(T\times \mathcal X\times \Theta)$, $w\in C(\mathcal X)$ and $q\in \R_{\ge 0}$.\par
Approximation of the set of initial conditions which reach $\mathcal X_T$,
\begin{align}
S_1=\{x\mid w(x)\ge 1+q(1-\alpha)\}
\end{align}
Approximation of the set of initial conditions which do not reach $\mathcal X_T$,
\begin{align}
S_2=\{x\mid w(x)\ge 1-q\alpha\}
\end{align}

Now, since $q\in \R_{\ge 0}$, it follows that $S_1\subset S_2$ and hence set of initial conditions of interest (BRS) to us is contained in $S_2$.


==> sections/sec_control.tex <==
\section{Control Synthesis}


